Impact of Distributed Rate Limiting on Load Distribution in a Latency-sensitive Messaging Service

The cloud's flexibility and promise of seamless auto-scaling notwithstanding, its ability to meet service level objectives (SLOs) typically calls for some form of control in resource usage. This seemingly traditional problem gives rise to new challenges in a cloud setting, and in particular a subtle yet significant trade-off involving load-distribution decisions (the distribution of workload across available cloud resources to optimize performance), and rate limiting (the capping of individual workloads to prevent global over-commitment). This paper investigates that trade-off through the design and implementation of a real-time messaging system motivated by Internet-of-Things (IoT) applications, and demonstrates a solution capable of realizing an effective compromise. The paper's contributions are in both explicating the source of this trade-off, and in demonstrating a possible solution.

==> loaddist.tex <==
\section{Iterative Load Distribution}
\label{app:loaddist}

In this section, we details the correlation-aware allocation
(within Step (2)) and the binary search of the profiling phase (within Step (3)). 

% \subsection{Achieving \textit{Max-min}}
% \label{app:mm}

% In the ``do-while loop" (line~10 to 24), we assign workload to each of the $k$ selected brokers.
% The assignment is done sequentially across the $k$ brokers (the ``for loop" from line~11 to 23). For each broker, we first determine the amount of workload, i.e., the $quota$, to be assigned to it (line~12 to 19). In this routine, we have to consider two separate conditions. Firstly, if the broker has not been assigned any workload yet (line~12), then its $quota$ would be the minimum value of the broker's residual capacity($broker_i.rcap$) and the fair share of the entire workload ($rate/k$). This $quota$ ensures each broker gets at least $rate/k$ workload, unless limited by the residual capacity. Within this condition, if unassigned workload is less than the $quota$ (line~14), then we have to migrate workload from other brokers (which currently have workload assignment larger than $rate/k$) in order to make this assignment reach the desired $quota$~\footnote{Meanwhile, we make sure migration does not reduce any brokers' assignment below $rate/k$.}. Secondly, if the broker already has previous assignment (line~17), then we know \textit{Max-min} has been taken care of. So its $quota$ only needs to consider residual capacity (accommodate as much workload as possible).

% However, by executing the ``for loop" once, we can not guarantee that the sum of the $k$ $quotas$ is equal to $rate$. For example, if we select two brokers ($k=2$), with
% $broker_1.rcap=25~kmsgs/s$ and $broker_2.rcap=10~kmsgs/s$, to handle a new topic with $rate = 30~kmsgs/s$. Then after the first time ``for loop", $broker_1.quota=15~kmsgs/$ and $broker_2.quota=10~kmsgs/s$, with $5~msgs/s$ remaining ($ua\_rate > 0$). This is the reason that we need the ``do-while" loop to wrap the ``for loop". With the extra check at line~24, we know when the ``for loop" has to be executed again, in which remaining workload is assigned.

\subsection{Correlation-aware allocation}
\label{app:ca}

Within Step (2), after $quotas$ (of the $k$ brokers) are set, the correlation-aware allocation is sequentially conducted to the $k$ brokers. For each broker, we first select the same proportion, which is the quotient of the broker's $quota$ and total workload $rate$, of publishers from each correlated group and then allocate them.

With this approach, we claim: for each allocation (to a single broker), the total workload of the selected publishers is equal to the $quota$, and message burst is decreased with the same proportion as the workload split. The proof is as follows:

\begin{proof}
Assume a topic has $n$ publishers, and each publisher has $1$ unit of workload. All the publishers belong to $m$ correlated groups with sizes $= \{n_1, ..., n_m\}$ subject to $\sum_{i=1}^{m} n_i = n $. Accordingly, the message arrival process of the new topic can be formed by $m$ independent bursts $= \{n_1, ..., n_m\}$. Given $broker_j$ with $quota = q_j$, then our allocation approach selects publishers from each correlated group with proportion $\frac{q_j}{n}$, and forms a set of publishers $P$. The total workload of $P$ is of the form

\begin{align*}
L(P) &= \sum_{i=1}^{m}\frac{q_j}{n}*n_i = \frac{q_j}{n}*\sum_{i=1}^{m}n_i = \frac{q_j}{n}*n = q_j
\end{align*}

, which means the the right amount of workload is selected. Besides, the message arrival process of $P$ also have $m$ bursts $= \{\frac{q_j}{n}*n_1, ..., \frac{q_j}{n}*n_m\}$. Hence, each original burst is split by $\frac{q_j}{n}$, which is the same proportion as the workload split, i.e., $\frac{L(P)}{n}$.
\end{proof}

With this approach, each allocation splits the burst in a manner that parallels the decrease of the respective token bucket size, which realizes the \textit{Correlation-awareness} principle.

% Note that in practice, because of the variance of event triggering, there are chances that multiple correlated groups partly or fully overlap, which aggregates their bursts. However, as introduced in Section~\ref{sec: bg}, identifying this inter-group correlation is computationally complex and impractical to realize in a distributed fashion. Hence, given only the intra-group correlation (from user inputs), our correlation-aware assignment is the simple but most effective approach to split burst.

\subsection{\textit{The binary search}}
\label{app:of}

Within Step (3), the binary search seeks to find the maximum subset of the newly-assigned publishers (from Step (2)) that a broker can accommodate without violating its SLO. Excess publishers are then returned to the Load Distributor

The binary search itself is a iterative procedure. In each iteration, we enable a subset of the newly-assigned publishers (while disabling the complementary set) and measure the resulting latency. If the result exceeds the latency threshold $\theta$ (defined in SLO contract), we shrink the subset by half. Otherwise, we enlarge the subset. Assuming $m$ publishers are assigned to a broker, then this binary search ends within at most $\log_{2}m$ steps. 

%Because each step requires certain amount of time to collect enough samples for a reliable latency measurement, the entire time complexity of the FIT function might be non-negligible.

In order to shorten the depth of this binary search, we use $[0.8*\theta, \theta]$ as an ``extended" latency threshold. This configuration relies on a fact that latency normally grows at increasing speed with load. Once latency has already approached the threshold, i.e., within $[0.8*\theta, \theta]$, then accommodating even a little amount of extra load is very likely to dramatically increase latency, thereby violating SLO. So during the binary search, once finding a subset of publishers with resulting latency within this ``extended" threshold, the procedure stops, and the complementary set of publishers (as the excess workload) is returned to the Load Distributor.







